Multiplex Heterogeneous Graph Convolutional Network

Heterogeneous graph convolutional networks have gained great popularity in tackling various network analytical tasks on heterogeneous network data, ranging from link prediction to node classification. However, most existing works ignore the relation heterogeneity with multiplex network between multi-typed nodes and different importance of relations in meta-paths for node embedding, which can hardly capture the heterogeneous structure signals across different relations. To tackle this challenge, this work proposes a Multiplex Heterogeneous Graph Convolutional Network (MHGCN) for heterogeneous network embedding. Our MHGCN can automatically learn the useful heterogeneous meta-path interactions of different lengths in multiplex heterogeneous networks through multi-layer convolution aggregation. Additionally, we effectively integrate both multi-relation structural signals and attribute semantics into the learned node embeddings with both unsupervised and semi-supervised learning paradigms. Extensive experiments on five real-world datasets with various network analytical tasks demonstrate the significant superiority of MHGCN against state-of-the-art embedding baselines in terms of all evaluation metrics.

==> tables/Notations.tex <==
\begin{table}[htbp]
\centering
\vspace{-2mm}
\caption{Main notations and their definitions.}
\label{table_notations}
\vspace{-2mm}
\begin{tabular}{c|c}
     \toprule
     Notation & Definition \\
     \midrule
     $\mathcal{G}$			& the input network\\
     $\mathcal{V}, \mathcal{E}$ & the node/edge set of $\mathcal{G}$\\
     $\mathcal{O},\mathcal{R}$	& the node/edge type set of $\mathcal{G}$\\
     $\mathbf{X}$		& the node attribute matrix of $\mathcal{G}$\\
     $\mathbf{H}$       & the node embedding\\
     $\mathbf{H}_v$       & the embedding of node v\\
     $\mathbf{A}$		& the adjacency matrix\\
     $\beta_r$            & the weight of sub-network adjacency matrix\\
     $\mathbb{A}$       & the adjacency matrix with meta-paths\\
     $d$			  	& the dimension of embeddings\\
     $n$			  	& the number of nodes\\
     $m$			  	& the dimension of attribute matrix\\
     $l$			    & the number of layers for GCN\\
     \bottomrule
\end{tabular}
\vspace{-3mm}
\end{table}

==> tables/ablation.tex <==
\begin{table}[t]
\begin{center}
\vspace{-2mm}
\caption{Ablation}
\vspace{-3mm}
\label{ablation}
\begin{threeparttable}
\setlength{\tabcolsep}{0.95mm}{}
% \scalebox{0.8}{
\begin{tabular}{c|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c|}{AMiner} & \multicolumn{2}{c|}{Alibaba} & \multicolumn{2}{c|}{IMDB} & \multicolumn{2}{c}{DBLP}\\
  & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 & Macro-F1 & Micro-F1 \\
\midrule
% \hline
MHGCN-r & 0.839 & 0.842 & 0.320 & 0.442 & 0.755 & 0.768 & 0.905 & 0.915\\
MHGCN-l & 0.843 & 0.850 & 0.330 & 0.447 & 0.754 & 0.755 & 0.931 & 0.937\\
\hline
\textbf{\system}  & \textbf{0.868} & \textbf{0.875} & \textbf{0.351} & \textbf{0.458} & \textbf{0.764} & \textbf{0.782} & \textbf{0.945} & \textbf{0.952} \\ 
\bottomrule
\end{tabular}
\end{threeparttable}
\end{center}
\vspace{-3mm}
\end{table}
